ASA -- The Adaptive Scheduling Algorithm

In High Performance Computing (HPC) infrastructures, the control of resources by batch systems can lead to prolonged queue waiting times and adverse effects on the overall execution times of applications, particularly in data-intensive and low-latency workflows where efficient processing hinges on resource planning and timely allocation. Allocating the maximum capacity upfront ensures the fastest execution but results in spare and idle resources, extended queue waits, and costly usage. Conversely, dynamic allocation based on workflow stage requirements optimizes resource usage but may negatively impact the total workflow makespan. To address these issues, we introduce ASA, the Adaptive Scheduling Algorithm. ASA is a novel, convergence-proven scheduling technique that minimizes jobs inter-stage waiting times by estimating the queue waiting times to proactively submit resource change requests ahead of time. It strikes a balance between exploration and exploitation, considering both learning (waiting times) and applying learnt insights. Real-world experiments over two supercomputers centers with scientific workflows demonstrate ASA's effectiveness, achieving near-optimal resource utilization and accuracy, with up to 10% and 2% reductions in average workflow queue waiting times and makespan, respectively.

==> math.tex <==
\subsection{Mathematical Analysis}

In this section, we formulate scheduling tradeoffs for different strategies when submitting workflows to HPC environments.
Libraries like \systemname are targeted to improve the resource usage of workflows, expressed as core-hours. 
Mathematically, the core-hours ($C$) is defined as $C = t * n$, where $t$ is the execution time (e.g. hours), and $n$ is the number of
cores assigned during execution. Hence for a workflow with $s$ stages,
the core-hours usage is calculated as the sum of core-hours used by each
stage as $C = \sum_{i=1}^{s}{t_i * n} $.

%\begin{align}
%\label{eq:ch_nehpc}
%C = \sum_{i=1}^{s}{t_i * n}
%\end{align}

Now, a workflow managed by \systemname allocates separate resources
to each stage of the workflow. Hence, each stage is assigned the number
of cores required for its execution. In addition, the checkpoint-restart
mechanism incurs an overhead that adds to the execution time of the stages.
So, core-hours usage for an \systemname managed workflow is given by:

\begin{align}
\label{eq:ch_ehpc}
C_{ehpc} = \sum_{i=1}^{s}{(t_i + CR_i) * n_i}
\end{align}

\noindent where, $CR_i$ represents the checkpoint-restart overhead for the
$i$-th stage. Using equations \ref{eq:ch_nehpc} and \ref{eq:ch_ehpc}, we can
derive that \systemname minimizes core-hours usage for a workflow iff:
\begin{align}
\label{eq:ch}
\sum_{i=1}^{s}{CR_i * n_i} < \sum_{i=1}^{s}{(n - n_i) * t_i}
\end{align}

\noindent Equation~\ref{eq:ch} shows that in order to provide better core-hours,
checkpoint-restart overheads must be \emph{less than} the core-hours gained for
the workflow execution. In other words, the total amount of core-hours gained in
workflow execution has to be more than the amount of core-hours lost due to \systemname
checkpoint-restart overheads. The result implies that the core-hours improvement
in \systemname is dependent on a number of external factors like the characteristics
of the workflow, the performance of the checkpoint-restart library, and the I/O
performance of the storage system on which the checkpoint images are written. 

In addition to minimizing the core-hours usage, \systemname also targets
improving the total turnaround time of a workflow. The turnaround time ($T$)
of a workflow is defined as:

\begin{align}
\label{eq:tt_nehpc}
T = t + q
\end{align}

\noindent where, $t$ is the execution time, and $q$ is the time to wait
in the queue for getting the requested resource allocation. Since \systemname
allocates resources separately to each stage of the workflow, the turnaround
time in \systemname is:

\begin{align}
\label{eq:tt_ehpc}
T_{ehpc} = \sum_{i=1}^{s}{(t_i + q_i + CR_i)}
\end{align}

\noindent where, $t_i$, $q_i$ and $CR_i$ are respectively the execution,
queue-wait and checkpoint-restart times for the $i$-th stage of the workflow.
Using equations \ref{eq:tt_nehpc} and \ref{eq:tt_ehpc}, we can derive that
the turnaround time in \systemname is better if:

\begin{equation}
\label{eq:tt_rel}
\begin{aligned}
\sum_{i=1}^{s}{(t_i + q_i + CR_i)} &< t + q \\
                                   &< \Big(\sum_{i=1}^{s}{t_i}\Big) + q
\end{aligned}
\end{equation}

\noindent Assuming the checkpoint-restart overhead is negligible i.e., $CR_i \approx 0$,
equation~\ref{eq:tt_rel} implies:

\begin{align}
\label{eq:tt}
\sum_{i=1}^{s}{q_i} &< q 
\end{align}

\noindent Equation~\ref{eq:tt} shows that \systemname improves the turnaround time
if the sum of individual queue wait times for each stage of the workflow is less
than the queue wait time of the complete workflow. 
In other words, \systemname achieves
better turnaround time if smaller jobs (stages of a workflow) have significantly less
wait time than larger jobs (the complete workflow). 
But as the queue wait time is a system parameter, controlled by the resource scheduler, \systemname cannot know when to submit jobs since it does not know the exact wait time.

\subsection{Challenge: Wait-Time prediction}

The clear tradeoffs seen in both approaches shown in Figure \ref{fig:ehpc_overview} and analyzed in the previous section, regard to the waiting time and resources usage (core-hours spent).
In one hand, submitting a large job for execution may have a long initial wait time, but no extra inter-stage waiting times.
Additionally, many resources will stay idle in sequential stages (where only one resource is needed).
At the expense of inefficient resource usage, these both characteristics allow for the minimum total workflow turn-around possible.

On the other hand, submitting many jobs separately (composing each workflow stage) has the advantage of efficiently using the resources. 
However with many extra inter-stage wait times, which increases the total turn-around time for the workflow, specially if it has many stages with different resource requirements.

A way to mitigate the increase in the total turn-around time while submitting many separate jobs would be to estimate the queue waiting time.
A pro-active submission strategy can use the waiting time estimations for a coming stage in a workflow, submitting its job during the execution of an ongoing stage, thus minimizing the waiting times between stages. 
However, depending on the estimation accuracy, three possibilities could happen: (i) perfect estimation, (ii) over-estimation, and (iii) under-estimation.

In (i), resource usage and total workflow execution time would be optimal.
In (ii), resource usage would be optimal, but a probable increase in total workflow execution time would be seen (though less than the current way achieved by \systemname).
In (iii), resources would be ready for use before they are actually needed, and depending on the policy used to mitigate the extra costs regarding this, both the resource usage and total workflow execution time could increase.
Some resource managers (like Slurm), allow for some constraints to be specified, including when a job may start execution in case some previous jobs have not finished.
